Towards Autonomous Grading In The Real World

In this work, we aim to tackle the problem of autonomous grading, where a dozer is required to flatten an uneven area. In addition, we explore methods for bridging the gap between a simulated environment and real scenarios. We design both a realistic physical simulation and a scaled real prototype environment mimicking the real dozer dynamics and sensory information. We establish heuristics and learning strategies in order to solve the problem. Through extensive experimentation, we show that although heuristics are capable of tackling the problem in a clean and noise-free simulated environment, they fail catastrophically when facing real world scenarios. As the heuristics are capable of successfully solving the task in the simulated environment, we show they can be leveraged to guide a learning agent which can generalize and solve the task both in simulation and in a scaled prototype environment.

==> ablation_study_tables.tex <==
\begin{table}[b]
\begin{tabular}{|l|l|l|l|l|}
\hline
down-sample factor {[}pix{]} & $2^1$ & $2^2$ & $2^3$ & $2^4$ \\ \hline
state space size             & $300^2$     & $150^2$ & $75^2$  & $38^2$     \\ \hline
params $*1e6$ in policy network (Yolo) $\downarrow$  & 3942     & 233     & 14.6     & 0.76     \\ \hline
volume left [ ] $\downarrow$            & 8.1    &  2.8      & \textbf{1.3}     & 11.1     \\ \hline
total reward [ ] $\uparrow$              & 1385     & 3002     & \textbf{4441}     & 2992     \\ \hline
mean height left [ ] $\downarrow$       & 22     & 8     & \textbf{4}     & 27     \\ \hline
\end{tabular}
\caption{state-space down-sampling parameter}
\label{Tab:table_1}
\end{table}

\begin{table}[!ht]
\begin{tabular}{|c|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{ablation net} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}P=Resnet,\\ V=Resnet\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}P=Resnet,\\ V=Yolo\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}P=Yolo,\\ V=Resnet\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}P=Yolo,\\ V=Yolo\end{tabular}} \\ \hline
volume left {[} {]} $\downarrow$        & 71   & 21   & \textbf{4}     & 18 \\ \hline
total reward {[} {]} $\uparrow$         & 7245 & 5630 & \textbf{10149} & 6601 \\ \hline
mean height left {[} {]} $\downarrow$   & 239  & 61   & \textbf{19}    & 51 \\ \hline
\end{tabular}
\caption{networks architecture ablation}

\label{Tab:table_2}
\end{table}

\begin{table}[!ht]

\begin{tabular}{|c|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{Gaussian scale factor ablation} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}4\end{tabular}} \\ \hline
volume left {[} {]} $\downarrow$        & 8.4   & 2.6   & \textbf{2.2}     & 11.3 \\ \hline
total reward {[} {]} $\uparrow$         & 2375 & 2620 & \textbf{3987} & 2191 \\ \hline
mean height left {[} {]} $\downarrow$   & 22.2  & 7.4   & \textbf{6.5}    & 30.1 \\ \hline
\end{tabular}
\caption{Gaussian masking ablation}

\label{Tab:table_3}
\end{table}

==> initial_image.tex <==



\begin{figure*}
 \centering
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/real_color_exp.png}
    %  \caption{Real RGB colormap}
     \label{fig:exp_real_color}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/real_heightmap_exp.png}
    %  \caption{Real Heightmap}
     \label{fig:exp_real_hmap}
 \end{subfigure}
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/simulated_heightmap_exp.png}
    %  \caption{Simulation Heightmap}z
     \label{fig:exp_sim_hmap}
 \end{subfigure}
    \caption{Comparison between a simulated environment and a real dozer before and after the grading action is preformed. top row is the rbg images captured by our experiment setup \ref{Real_world_comparison}. middle row is the, heigh-map. both top and middle observations are projected to world coordinates. bottom row is the same state, as it was generated by our simulator. \rc{add a-e and make larger individual images}. (a) state space for initial state. (b-e) states after actions taken in simulated environment and in real one. This figure depicts the resemblance in simulated and real height-maps in the grading task. }
    \label{fig:sim2real_all}
\end{figure*}

==> intorduction_oren.tex <==
\section{Introduction} \label{Introduction}

Recent years have seen a dramatic rising demand in the construction industry. Dozers play a key role in each and every construction site and are the go-to machinery for many tasks. While manual dozing is a well established profession, it suffers from shortage in experienced drivers which induces longer construction times and higher costs. our work focuses on automation of the grading task where a dozer (see robotic example in \cref{fig:sim2real_all}) is confronted with an uneven plot of land. The dozer is equipped with a blade and by pushing around the sand/gravel, it is required to bring the plot to a target height. 

Similar to other real life robotics solutions, grading suffers from two major challenges. 
first, we have a partially observed system due to missing/noisy sensory information and limited field-of-view of the agent. 
second, obtaining diverse real world experience is expensive and exploration for pure RL methods might be dangerous.

On one hand, path-planning rule-based approach \cite{hirayama2019path} can create grading plan without expensive data collection but fails when encountered with real life partially observed information. on the other hand, Reinforcement learning (RL) relies on trial and error shown to handle partially observed system but suffers from its necessitates of large amounts of real-world data.

% The autonomous grading task was recently tackled from a path-planning rule-based approach \cite{hirayama2019path}. The system creates a grading plan by selecting goal-points the agent is required to reach. They considered various heuristics for how to approach the sand piles. However, we show that while this approach solves the expensive data collection drawback it fails when encountered with real life partially observed information.

% Reinforcement learning (RL) offers a different solution, relying on trial and error learning instead
% of accurate modeling to construct an effective controller. RL with expressive function approximation, i.e. deep RL,
% has further shown to automatically handle high dimensional inputs such as images. However, it necessitates large amounts of real-world data.

In this paper, we combine both approaches to tackle the two challenges. we first, introduce a first order simulation based on numerical understanding on sand piles to help us obtain diverse real life experience. Sencond, we use rule-based approach \cite{hirayama2019path} to initialize our learned agent policy. lastly, we use domain adaptation and domain randomization techniques to decrease the sim2real gap. 
Our main contributions are: \\
\textbf{(1)} We formalize the task of grading as that of sequential decision making \yg{should we keep?}\chen{have other works properly defined this task in a way that makes this meaningless? otherwise its a "contribution" that can give bonus points.}. We define the properties such as states, observations and actions.\\
\textbf{(2)} We create a physically realistic simulation environment for training and evaluation of both heuristics and learning-based agents.\\
\textbf{(3)} We show that training agents using privileged ML techniques can be used to overcome the limitations of standard methods for autonomous grading. \\
\textbf{(4)} We create a scaled prototype environment and validate our claims in the real world.

==> results_old.tex <==

\section{Experiments} \label{sec: experiments}
To demonstrate our method and the efficacy of our algorithms, we compared them on three types of problems, as outlined in Figure \ref{fig:scenario_examples} and explained in Section \ref{Problem Formulation}. We trained our policy model with $8$ different algorithms and focused our comparison on $4$ metrics. 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/example_figures/snp_traj_comparison_105.png}
         \caption{\textbf{SnP, $R_T=1554$}}
         \label{fig:snp_traj}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/example_figures/bc_traj_comparison_105.png}
         \caption{\textbf{BC}, $R_T=1555$}
         \label{fig:bc_traj}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/example_figures/rl_traj_comparison_105.png}
         \caption{\textbf{RL+BC+CL}, $R_T=1556$}
         \label{fig:rl_traj}
     \end{subfigure}
     \hfill
        \caption{Comparison between trajectories from different policies for the continuous problem. Each triangle is another action and the lines indicate the paths between these actions. Each row shows a different policy (\textbf{SnP}, \textbf{BC}, \textbf{RL+BC+CL}) and each column a different stage of the episode. $R_{T}$ is the total reward.}
        \label{fig:trajectory_example}
\end{figure}
\input{results_table}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\linewidth]{images/example_figures/rl_training_std.png}
    \caption{ Example of RL Reward for our top policies during validation on initial scenarios (while training). Here, the mean reward was calculated during training on $50$ different initial episodes. \textbf{RL+BC+CL} reaches the best overall reward \textbf{faster} than other policies. In addition, \textbf{RL+CL} continues to learn throughout all the steps. Note that the std. is large due to a variety of scenarios (each scenario can reach a different reward depending on the initial number of sand piles).    }
    
    \label{fig:rl_loss}
\end{figure}

 \begin{figure}
     \centering
     \begin{subfigure}[b]{0.113\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sigma/gaussian_dist_1.png}
         \caption{$\lambda_\sigma=1$}
         \label{fig:sigma_coeff1}
     \end{subfigure}
     \begin{subfigure}[b]{0.113\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sigma/gaussian_dist_2.png}
         \caption{$\lambda_\sigma=2$}
         \label{fig:sigma_coeff2}
     \end{subfigure}
     \begin{subfigure}[b]{0.113\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sigma/gaussian_dist_3.png}
         \caption{$\lambda_\sigma=3$}
         \label{fig:sigma_coeff3}
     \end{subfigure}
     \begin{subfigure}[b]{0.128\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sigma/gaussian_dist_4.png}
         \caption{$\lambda_\sigma=4$}
         \label{fig:sigma_coeff4}
     \end{subfigure}
        \caption{Gaussian mask for different coefficients of $(\sigma_x, \sigma_y)$. Higher numbers indicate pixels with a height probability of being chosen}
        \label{fig:sigma_coeff_all}
\end{figure}

 
For the purpose of evaluation, we ran $50$ runs for each scenario type generated from the same distribution and compared the mean result for each metric. Each initial state had a different number of sand piles, set up in a lattice format, and the dozer was positioned facing the piles. All the algorithms were calculated on the same scenarios to ensure a fair comparison.

Autonomous off-road planning is complex and, specifically, the grading assignment does not have classic solvers for comparison. We, therefore, compared our results to the \textbf{SnP} heuristic that is based on \cite{hirayama2019path}, who used experienced expert drivers and mimicked their behaviour.

\subsection{AGPnet Results} 

We show our results on all metrics in Table \ref{tab:all_results}.

The results of the majority of our approaches are on par with the \textit{baseline} heuristic. We found that our combined algorithms approach (RL+BC+CL) outperforms the heuristic in terms of important metrics and overall reward. 
In our approaches, the agent learns from experienced rule-based algorithms similar to other BC models but also trains on online policies allowing for exploration. 
In addition, we enhanced the policies' ability to detect important features in the state space by adding a CL loss (\textbf{CL}), and the final EGO-Gaussian masking layer in the policy ensures our agent does not explore irrelevant areas.

The data set used to train the \textbf{BC} policies included $150$ episodes, each with a range of states.

In Figure \ref{fig:trajectory_example}, we show a comparison between the trajectories for $3$ agents (\textbf{Snp}, \textbf{BC} and \textbf{RL+BC+CL}). It is evident that the \textbf{BC} algorithm manages to mimic the \textbf{SnP} heuristic well, and that, although it never trained on this episode, it rarely chooses unwanted decisions (generalization capabilities). The \textbf{RL+BC+CL} trajectory has less actions and manages to grade more soil at an earlier step (see left column). Moreover, this policy reaches an overall higher reward and lower final height.

\subsection{Ablation Study}\label{Ablation_study}
\input{ablation_study_tables}

Our ablation study considered various network architectures, Gaussian masking coefficients and down-sampling. We expand on each architecture below.

\textbf{Network architecture}: We examined two architectures for the policy and value neural network: Resnet18 \cite{He_2016} and Yolo lite \cite{Huang_2018}. Ablations show that for the policy network, Yolo lite outperforms Resnet18, and for the value network, Resnet18's performance was superior (\ref{Tab:table_2}).
 
\textbf{Gaussian masking}: We added the Gaussian masking to the action space selection. This was done to allow the agent to learn to take actions that are closer to the current location if the received reward is beneficial. Without this mask, actions further away from the current location were selected, leading to an increase in the episode time and to sub-optimal performance. 
We examined \textit{four} values of the sigma factor that was applied to generate the mask. A Gaussian sigma factor is the divisor of $(\sigma_x,\sigma_y)$ in the Gaussian mask that was applied in the action space.
$(\lambda_{\sigma_x}, \lambda_{\sigma_y}) = (1,2,3,4)$, where "4" masks out further away pixels in the action space and "1" alleviates this restriction. please refer to fig \ref{fig:sigma_coeff_all}, Results show that the optimal value is $3$. (see \ref{Tab:table_3} \label{Gaussian_masking}).


    
\textbf{Down-sampling}: \label{down-sampling} As noted above, the selected action is sampled out of the learnt distribution of the pixels in the agent's FOV, a representation that might be of high resolution. We examined lowering the state space representation dimension to decrease both the memory footprint and the task time. We examined four exponential values for the state space down-sampling parameter, i.e., $2^{(1,2,3,4)}$. This was done on the RL+BC+CL problem. Table \ref{Tab:table_1} depicts the results when the parameter was set to $2^3$. This configuration achieves the best results for removing the mean volume and height in the grading problem as well as the best rewards from the simulation environment. The number of parameters in the policy network is fairly small w.r.t. its performance. All these parameters are unit-less, as they were all normalized by some constant factor to allow fair comparison.

\input{conclusion}





==> results_table.tex <==

\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|llllllllll|}
\hline
\multicolumn{1}{|l|}{\textbf{scenario type}} &
  \textbf{metric} &
  \textbf{BC} &
  \textbf{BC+CL} &
  \textbf{RL} &
  \textbf{RL+BC} &
  \textbf{RL+BC+CL} &
  \textbf{RL+BC+CL+res} &
  \textbf{RL+BC+res} &
  \textbf{RL+CL} &
  \textbf{RL+res} &
  \textbf{SnP} \\ \hline
\multirow{4}{*}{\textbf{Init}} &
  \textbf{volume $\downarrow$} &
  0.63 &
  21.97 &
  1.03 &
  0.57 &
  0.25 &
  1.49 &
  0.54 &
  \textbf{0.07} &
  37.66 &
  0.36 \\
 &
  \textbf{height $\downarrow$} &
  2.06E-04 &
  7.20E-03 &
  2.71E-04 &
  1.76E-04 &
  \textbf{7.12E-05} &
  4.35E-04 &
  1.52E-04 &
  2.19E-05 &
  9.75E-03 &
  1.15E-04 \\
 &
  \textbf{time $\downarrow$} &
  5024 &
  6566 &
  14464 &
  14326 &
  12975 &
  13778 &
  12263 &
  11140 &
  8166 &
  \textbf{3278} \\
 &
  \textbf{reward $\uparrow$} &
  1478 &
  930 &
  1714 &
  1916 &
  2687 &
  \textbf{3279} &
  2923 &
  3132 &
  741 &
  1934 \\ \hline
\multirow{4}{*}{\textbf{Continuous}} &
  \textbf{volume $\downarrow$} &
  15.04 &
  46.53 &
  0.70 &
  0.36 &
  0.29 &
  0.91 &
  0.74 &
  0.16 &
  23.95 &
  \textbf{0.12} \\
 &
  \textbf{height $\downarrow$} &
  4.10E-03 &
  1.28E-02 &
  1.87E-04 &
  \textbf{9.92E-05} &
  8.63E-05 &
  2.63E-04 &
  2.08E-04 &
  4.98E-05 &
  5.95E-03 &
  3.74E-05 \\
 &
  \textbf{time $\downarrow$} &
  6232 &
  7282 &
  11455 &
  15775 &
  12857 &
  14466 &
  14878 &
  8864 &
  7993 &
  \textbf{3451} \\
 &
  \textbf{reward $\uparrow$} &
  1584 &
  712 &
  1681 &
  2910 &
  2271 &
  \textbf{4101} &
  3365 &
  3123 &
  772 &
  2585 \\ \hline
\multirow{4}{*}{\textbf{Edge}} &
  \textbf{volume $\downarrow$} &
  0.25 &
  4.65 &
  1.22 &
  0.42 &
  0.30 &
  2.16 &
  0.53 &
  0.10 &
  33.37 &
  \textbf{0.05} \\
 &
  \textbf{height $\downarrow$} &
  7.74E-05 &
  1.81E-03 &
  3.49E-04 &
  1.20E-04 &
  \textbf{8.89E-05} &
  6.33E-04 &
  1.53E-04 &
  3.39E-05 &
  8.47E-03 &
  1.42E-05 \\
 &
  \textbf{time $\downarrow$} &
  4657 &
  5670 &
  10981 &
  12065 &
  5993 &
  8333 &
  9802 &
  8468 &
  4633 &
  \textbf{3094} \\
 &
  \textbf{reward $\uparrow$} &
  939 &
  475 &
  1624 &
  2447 &
  \textbf{3690} &
  1901 &
  2528 &
  3512 &
  345 &
  2791 \\ \hline
\end{tabular}%
}
\caption{All the results for our algorithms, including the SnP heuristic, BC, RL and hybrid methods. Our hybrid methods achieve better results on the main metric (height) and the overall reward. Results are mean over 50 i.i.d runs.}
\label{tab:all_results}
\end{table*}

==> table_params.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


% paramaters for bc training - 
\begin{table}[ht]
\centering
{%
\begin{tabular}{|c|c|}
\hline
learning rate         & 1.00E-05   \\ \hline
train batch size      & 120        \\ \hline
validation batch size & 40         \\ \hline
validation percentage & 5          \\ \hline
downsample factor     & 3          \\ \hline
gaussian factor       & 3          \\ \hline
number of episodes    & 150        \\ \hline
use\_cl               & True/False \\ \hline
\end{tabular}%
}
\caption{Parameters for training BC algorithms (use\_cl is True if training with CL and False otherwise)}
\label{tab:bc_params}
\end{table}



% parameters for training rl 
\begin{table}[ht]
\centering
{
\begin{tabular}{|c|c|}
\hline
learning rate        & 1.00E-03   \\ \hline
downsample factor    & 3          \\ \hline
gaussian factor      & 3          \\ \hline
loss update interval & 100        \\ \hline
minibatch size       & 50         \\ \hline
value loss coefficient    & 0.0001     \\ \hline
gamma                & 0.95       \\ \hline
bc loss coefficient  & 1000       \\ \hline
scenario type        & random     \\ \hline
$\lambda_t$      & 0.05       \\ \hline
$\lambda_h$      & 5          \\ \hline
$\lambda_v$      & 10         \\ \hline
$\lambda_d$      & 10         \\ \hline
$\lambda_f$      & 1         \\ \hline
use\_cl               & True/False \\ \hline
use\_bc               & True/False \\ \hline
use\_res              & True/False \\ \hline
\end{tabular}}
\caption{Parameters for training RL algorithms. use\_cl, use\_bc and use\_res are boolean parameters that indicate which training was performed. }
\label{tab:rl_params}
\end{table}
